Entity-Graph Enhanced Cross-Modal Pretraining for Instance-level Product Retrieval

Our goal in this research is to study a more realistic environment in which we can conduct weakly-supervised multi-modal instance-level product retrieval for fine-grained product categories. We first contribute the Product1M datasets, and define two real practical instance-level retrieval tasks to enable the evaluations on the price comparison and personalized recommendations. For both instance-level tasks, how to accurately pinpoint the product target mentioned in the visual-linguistic data and effectively decrease the influence of irrelevant contents is quite challenging. To address this, we exploit to train a more effective cross-modal pertaining model which is adaptively capable of incorporating key concept information from the multi-modal data, by using an entity graph whose node and edge respectively denote the entity and the similarity relation between entities. Specifically, a novel Entity-Graph Enhanced Cross-Modal Pretraining (EGE-CMP) model is proposed for instance-level commodity retrieval, that explicitly injects entity knowledge in both node-based and subgraph-based ways into the multi-modal networks via a self-supervised hybrid-stream transformer, which could reduce the confusion between different object contents, thereby effectively guiding the network to focus on entities with real semantic. Experimental results well verify the efficacy and generalizability of our EGE-CMP, outperforming several SOTA cross-modal baselines like CLIP, UNITER and CAPTURE.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> ex_conclusion.tex <==
\section{Conclusion}\label{sec:conclu}
In this paper, we present the first effort on extending canonical intra-/cross-modal retrieval to a more generalized setting, i.e., weakly-supervised multi-modal instance-level product retrieval, which has wide application potential in the E-commerce industry.
We contribute Product1M, which is one of the largest multi-modal retrieval datasets as well as the first one specifically tailored for instance-level retrieval. 
% We organize Product1M carefully and adopt several metrics to evaluate the performance and robustness of a retrieval algorithm comprehensively.  
Aside from that, we propose a novel hybrid-stream transformer, named CAPTURE, that excels in capturing the potential synergy between data of different modalities. 
Moreover, we overcome the unmatched issue incurred by the inappropriate pretext task by enforcing cross-modal contrastive learning between multi-modal features.
Extensive experiments demonstrate that our CAPTURE surpasses the SOTA cross-modal pretraining models in terms of all metrics by a large margin. 
We hope the proposed Product1M, CAPTURE, and solid baselines will spur further investigation into a more reliable and flexible retrieval system.
\section{Acknowledgement}
This work was supported in part by National Key R&D Program of China under Grant No.2018AAA0100300, National Natural Science Foundation of China (NSFC) under Grant No.U19A2073 and No.61976233, Guangdong Province Basic and Applied Basic Research (Regional Joint Fund-Key) Grant No.2019B1515120039, Guangdong Outstanding Youth Fund (Grant No.2021B1515020061), Shenzhen Fundamental Research Program (Project No.RCYX20200714114642083, No.JCYJ20190807154211365).


==> ex_experiment.tex <==
\section{Experiments}
\label{sec_exp}
% We first elaborate on the implementation details in Section \ref{sec_implement}.
% Then we compare our multi-modal retrieval scheme with text-based and image-based retrieval in Section \ref{sec_cross_comparison}.
% We further verify the significance of the relation modeling of multi-modal inputs by comparisons with variants of CAPTURE and several prevailing models in Section \ref{sec_relation_ablation}.
% In Section \ref{sec_imagelevel_comparison}, we illustrate the challenges of instance-level retrieval in comparison to image-level and single-product retrieval.
% We verify the generalization capacity of our model to unseen categories in Section \ref{sec_generalize}.




% \FIXME{
% Due to the lack of annotated bounding boxes, it is difficult to locate the instance in the suit images. Image-level feature will be concentrated on a salient product and thus casuing retrieval results contain many images relative to this salient product. Such method will ignore many other products in the suit images. 
% So it's a good choice to generate the bounding box from the multi-product image and using bounding boxes which contain one product for retrieval will improve the performance.
% However, When using detectors trained on other annotated datasets, many irrelevant objects in the background will be selected as bounding box, so for generating accurate bounding box, it's necessary to train the detector on our dataset. 
% To generate some coarse annotations, we first achieve the foreground segmentation from the single-product image which contain a simple background and only singe product.
% Then use the copy and paste method to create synthesized suit images.
% With these synthesized images and  bounding box annoatation, we feed them to train a Region Porposal Network(RPN)  for high-quality proposals.
% }





\subsection{Implementation Details}
\label{sec_implement}
We attach RPN to a ResNet-50 \cite{he2016deep} backbone pre-trained on ImageNet and follow the training schedule in \cite{ren2015faster}.
We use the BERT \cite{devlin2018bert} to initialize the linguistic transformer of our CAPTURE. 
% The Lower transformer for capture separate modal information is iterated for $L=6$ times and the co-attention transformer is iterated for $K=6$ times, the upper transformer is iterated for $H=3$ times. 
The number of the Text/Visual Transformer, Text/Visual Cross-Transformer, and Co-Transformer is set to $L=4, K=4,$ and $H=4$, respectively, which adds up to 12 transformer layers.
We set the hidden state size of CAPTURE and other baselines to 768 for a fair comparison. 
We separately attach a 512-d fully connected layer after Co-Transformer and Text/Visual Transformer for masked multi-modal learning and cross-modal contrastive learning. 
The concatenation of the features from these two layers results in a 1024-d feature vector for retrieval, which is also the same for other baselines.
The maximum sequence length for the sentence is set to 36. 
We train CAPTURE with a total batch size of 128 for 10 epochs on 4 RTX 2080 GPUs. 
We use Adam \cite{kingma2014adam} optimizer with an initial learning rate of 1e-4 and a linear learning rate decay schedule is adopted. 
Temperature parameter $\tau$ is set to 0.07.
%testing details
At inference, CAPTURE takes as input the texts and proposal-wise features to generate instance features.
For a fair comparison with other baselines, we adopt the same training procedure and evaluation protocol in all experiments unless otherwise stated and we use the same augmentation-based RPN for the baselines in Table \ref{tab_performance}.
More details can be found in the Supplementary Materials.

\section{RPN Training Details}
We utilize a simple yet effective data augmentation scheme to train a Region Proposal Network (RPN) based on the single-product images. 
We select about 5000 images with simple background from single-product images.
Then GrabCut \cite{Meng2014GrabCut} method is adopted to extract the foreground masks of these single-product samples.
These masks are used to generate the bounding box pseudo-labels and are pasted onto the background images from Place365 \cite{zhou2017places} following the copy-and-paste strategy in \cite{dwibedi2017cut}. 
More than 40,000 synthetic images are generated in this step and 
Figure ~\ref{fig:fig_syn_images} showcases some synthesized images by copy-and-paste augmentation. 
% We use generated synthetic images to train a Region Proposal Network and select the RPN model whose Average Recall (AR) achieved to 96\%as our basic RPN. 
We fix the parameters of backbone pre-trained on ImageNet and train RPN for 5 epochs on the synthesized images. 
During training, we adopt an SGD optimizer with a momentum of $0.9$ and a weight decay of $1\times 10^{-4}$. 
The mini-batch size is set to $16$.
The input images are resized into $11$ scales ranging from $480$ to $800$ with a step size of $32$. 
% Our RPN achieves $96$\% Average Recall and 
The detection results are visualized in Figure \ref{fig:fig_RPN_box}.

\subsection{More Retrieval Details of CAPTURE}
We keep the number of input regions between 10 to 36 by selecting regions with predicted confidence higher than a threshold as in \cite{lu2019vilbert}. 
The features of region extracted by the RoIAlign are then flatten and fed into CAPTURE.
The transformer blocks in CAPTURE have hidden state size of 768 with 8 attention heads.
During retrieval, we compute cosine similarities between each box query with single-product samples and rank all retrieval single-product results according to their similarities. 
The top-$N$ samples are returned as the retrieval results.
Fig~\ref{fig:fig_retrieval_results} shows more retrieval results by CAPTURE. 

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{images/retrieval_results.png}
    \caption{More retrieval visualizations of CAPTURE. Multi-product query images are on the left. Correct retrieval images are highlighted in green boxes while the incorrect ones are highlighted in red boxes. The captions of retrieved samples are omitted
 for simplicity.}
    \label{fig:fig_retrieval_results}
\end{figure*}


\noindent\textbf{Evaluation Metrics.}
We adopt Precision ($\mathrm{Prec}@N$), mean Average Precision ($\mathrm{mAP} @ N$) and mean Average Recall ($\mathrm{mAR} @ N$) as our evaluation metrics, among which $\mathrm{Prec}@N$ and $\mathrm{mAP} @ N$ are widely used in the retrieval literature \cite{weyand2020GLDv2,CGW17}. 
Since exhaustively retrieve every single product is unnecessary and impractical in many scenarios, we report $\mathrm{mAP}$, $\mathrm{mAR}$, and $\mathrm{Prec}$ for $N = 10, 50, 100$.
The details of evaluation metrics can be found in the Supplementary Materials.

\subsection{Evaluation Metrics}
We adopt Precision ($\mathrm{Prec}@N$), mean Average Precision ($\mathrm{mAP} @ N$) and mean Average Recall ($\mathrm{mAR} @ N$) as our evaluation metrics.
$\mathrm{Prec} @ N$ evaluates the average accuracy of the top-$N$ predictions per image and is widely used in the retrieval literature.
$\mathrm{Prec} @ N(q)$ is computed as follows:
\begin{equation}
    \mathrm{Prec}@N(q) = \frac{1}{N}\sum_{i=1}^N \mathrm{acc}_q(i),
\end{equation}
where $\mathrm{acc}_q(i)$ is a binary indicator function that returns $1$ when the $i$-th prediction is correct for the $q$-th query and $0$ otherwise. 
$\mathrm{mAP} @ N$ is computed as the average $\mathrm{AP@}N$ per image, where $\mathrm{AP@}N(q)$ is computed as follows:
% \begin{equation}
%     \mathrm{mAP} @ N=\frac{1}{Q} \sum_{q=1}^{Q} \mathrm{AP} @ N(q),
% \label{eq_map}
% \end{equation}
% where
\begin{equation}
    \mathrm{AP@} N(q)=\frac{1}{\min \left(m_{q}, N\right)} \sum_{k=1}^{N} \mathrm{P}_{q}(k) \mathrm{rel}_q(k),
\label{eq_ap}
\end{equation}
% $Q$ is the number of multi-product query images, 
where $m_q$ is the total number of ground truth images, i.e., corresponding single-product images that appear in the $q$-th query image, $P_q(k)$ is the precision at rank $k$ for the $q$-th query, and $\mathrm{rel}_q(k)$ is a binary indicator function that returns $1$ when the $k$-th prediction is correct for the $q$-th query and $0$ otherwise. 
To evaluate the recall of instance-level retrieval results, we propose metric $\mathrm{mAR} @ N$, which can be computed as the average $\mathrm{AR@}N$ per image. 
% as follows:
% \begin{equation}
%     \mathrm{mAR} @ N=\frac{1}{Q} \sum_{q=1}^{Q} \mathrm{AR} @ N(\mathrm{q}),
% \label{eq_mar}
% \end{equation}
% where
$\mathrm{AR@}N(q)$ is computed as follows:
% \begin{equation}
%     \mathrm{AR@} N(q) = \frac{1}{\sum_{c=1}^C \mathbbm{1}_q(c)} \mathrm{count}(RETR^q),
% \end{equation}
\begin{equation}
    \mathrm{AR@}N(q) = \frac{1}{C_q}\sum_{c=1}^{C}\mathbbm{1}_c(q)\mathrm{min}(1, \frac{RETR^q_c}{\mathrm{min}(\lfloor r_q^c \cdot N \rfloor, G_c)})
\end{equation}
where $C$ is the total number of single-product categories in the \textit{gallery} set, $C_q$ equals to the number of existing categories in the $q$-th query, $\mathbbm{1}_c(q)$ is a binary indicator function that returns 1 when class $c$ exists in the $q$-th query, $RETR^q_c$ is the number of retrieved products belonging to class $c$ for the $q$-th query, $G^c$ is the number of ground truths belonging to class $c$ in the \textit{gallery} set, $r_q^c$ is the instance ratio\footnote{For instance, for a 2A+3B query image, $r_q^A=0.4$ and $r_q^B=0.6$.} of category $c$ in the $q$-th query, and $\lfloor\cdot\rfloor$ is rounding operation. 
As per the equation, $\mathrm{AR@}N(q)$ takes the category distribution into account, i.e.,
the inclusion of instance ratio is informative for evaluating both the correctness and diversity of a retrieval algorithm and guarantees that some trivial results are not overestimated\footnote{For a 2A+3B query image and $N=100$, $\mathrm{AR@}100(q)$ returns 0.51 and 1.0 for retrieval results 1A+99B and 40A+60B, respectively.}.


\subsection{Weakly-Supervised Instance-Level Retrieval}
\label{sec_main_results}
We compare CAPTURE with several intra- and cross-modal baselines and the results are shown in Table \ref{tab_performance}. 

\noindent \textbf{Intra-Modal Schemes.}
% Intra-modal retrieval approaches perform matching search between homogeneous data. 
% However, they are sub-optimal for our proposed task since they are subject to single modality of data and thus lack the modeling of cross-modal relations. 
We compare our method to two intra-modal schemes including \textit{Image-based} and \textit{Text-based} schemes. 
For image-based retrieval, we stack the Visual Transformer layer described in Section \ref{sec_CAPTURE_arch} and adopt the same image input and pretext task, i.e., Masked Region Prediction as CAPTURE.
For text-based retrieval, we stack the Text Transformer layer and use only the text input and Masked Language Modeling pretext task. 
We further double the depth of these two models to 24 layers to keep the same amount of parameters as CAPTURE.
It turns out that these two schemes are lagging far behind since they are subject to data of single modality, which suggests that the modeling of the relations between multi-modal data is indispensable.
We provide more experiment results to validate this point in Section \ref{sec_layer_ablation}.

% we \FIXME{ utilize ResNet50 to extract the image feature and train with the triplet loss, in which the positive pair and the negative pair is constructed according to the text similarity. ***}.
% we utilize a ResNet-50 backbone pre-trained on ImageNet to extract the image features supervised by the triplet loss \cite{hermans2017defense}, in which the positive and negative pairs are constructed according to the text similarity.

\noindent\textbf{Cross-Modal Schemes.}
We compare CAPTURE to several prevailing self-supervised cross-modal pretraining methods in Table \ref{tab_performance}, including SOTA single-stream and two-stream Vision-language models as well as a SOTA zero-shot classification model, i.e., CLIP \cite{radford2021learning}.
The CLIP* baseline refers to a CLIP-like architecture that uses separate transformers to encode image and text and is trained with a contrastive objective. 
Notably, CAPTURE outperforms all these baselines in all three metrics for instance-level retrieval.
Two-stream models, i.e., ViLBERT \cite{lu2019vilbert}, LXMERT \cite{tan2019lxmert} and CLIP*, are generally worse than single-stream ones, which suggests that the fusion mode of multi-modal features is one of the critical factors.
We attribute the superior performance of CAPTURE to its hybrid-stream architecture and we study the impact of different layer types in Section \ref{sec_layer_ablation}. 



% \begin{table}[]
% \label{tab:loss_ablation}
% \centering
% \setlength{\belowcaptionskip}{-0.6cm}
% % \footnotesize
% % \tabcolsep 0.02in 
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{cc|ccc|c}
% \toprule[1pt]
% % \multirow{2}{*}{\#} & 
% \multirow{2}{*}{\makecell{MRP+MLM}} &
% \multirow{2}{*}{\makecell{ITM}} &
% \multicolumn{3}{c|}{Cross-modal Contrastive} & 
% % \multirow{2}{*}{ mAP@100} & 
% % \multirow{2}{*}{ mAR@100} & 
% \multirow{2}{*}{mAP@100} \\ 
%  & & 
%  Cross- & 
%  Co- &
%  Txt\&Vis- &
%   \\ 
% \midrule[1pt]
% % 0& &&\checkmark&&&&&& \\
%  \checkmark&&&&      & 72.08\\
%  \checkmark& \checkmark &&&    &  70.27 \\
%  \checkmark&  & \checkmark&&  & 28.98  \\
%  \checkmark&  &&\checkmark&   & 28.59  \\
%  \checkmark&  &&&\checkmark    & 74.63   \\
% %  \checkmark&  & \checkmark&&&\checkmark&  68.38   & 26.63   &   66.30 \\

% \toprule[1pt]
% \end{tabular}
% }
% % \vspace{-2mm}
% \caption{The impact of different pretext tasks and cross-modal contrastive loss.}
% \label{tab:loss_ablation}
% \end{table}


\begin{table}[]
\label{tab:loss_ablation}
\centering
% \setlength{\belowcaptionskip}{-0.6cm}
\footnotesize
% \tabcolsep 0.02in 
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|c}
\toprule[1pt]
% \multirow{2}{*}{\#} & 
\#&Masked & ITM & CTR & Concat & mAP/mAR/Prec \\


\midrule[1pt]
% 0& &&\checkmark&&&&&& \\
1& \checkmark&&&     & 72.1 / 28.9 / 72.7 \\
2& \checkmark& & &  \checkmark    
 & 71.9 / 28.5 / 72.9 \\
3& \checkmark& \checkmark &&    &  70.2 / 27.1 / 70.2 \\
4&  \checkmark&  & \checkmark &   &  73.3 / 29.1 / 73.2  \\
%   \checkmark&  & \checkmark & \checkmark   
%   &  69.3/27.6/68.4  \\
5& \checkmark&  &\checkmark&\checkmark    & \textbf{74.6} / \textbf{30.1} / \textbf{73.9}\\
%  \checkmark&  & \checkmark&&&\checkmark&  68.38   & 26.63   &   66.30 \\

\toprule[1pt]
\end{tabular}
}
% \vspace{-2mm}
\caption{The impact of different pretext tasks and cross-modal contrastive loss. Evaluation for $N=100$. `Masked' stands for two masked multi-modal pretext tasks, i.e., MLM and MRP. `CTR' stands for cross-modal contrastive loss.}
\label{tab:loss_ablation}
\end{table}






\subsection{Impact of Pretext Tasks and Contrastive Loss}
\label{sec_pretext_ablation}
As shown in Table \ref{tab:loss_ablation}, ITM will hurt the accuracy of instance-level retrieval (\#1 vs \#3), since it gives rise to mismatch samples, which might be detrimental to the fine-grained understanding of a multi-product image. 
% However, we find that when applied to all three types of transformer layers, it slightly drops the performance. 
% We conjecture this is because the features at the deeper layers are more similar and the contrastive loss is of little help.
We apply the cross-modal contrastive loss at the Text/Visual Transformer layer to align the representations of image and text, which further benefits the learning of consequent layers. 
The inclusion of contrastive loss encourages our model to maximizes the feature similarity of positive pairs, which improves all three metrics by 1.2, 0.2, and 0.5, respectively (\#1 vs \#4), and we find it of little help when added to the deeper layers. 
% Moreover, we study the impact of the proposed cross-modal contrastive loss when applied on different layers of CAPTURE.
% Surprisingly, when applied on the Cross- and Co-Transformer layer, the mAP drops significantly. 
% Nevertheless, when applied on the Text- and Visual-Transformer layer, it boosts mAP@100 from 72.08 to 74.63. 
Moreover, after concatenating the features from the Text/Visual Transformer with that from the Co-Transformer for retrieval, it further improves all three metrics by 1.3, 1.0, and 0.7, respectively (\#4 vs \#5). 
However, we find this concatenation operation will slightly degrade the performance of the model without contrastive loss (\#1 vs \#2), which suggests that the improvement mainly comes from the contrastive loss instead of the operation itself.


\begin{table}[h]
\centering
\footnotesize
\setlength{\belowcaptionskip}{-0.5cm}
% \tabcolsep 0.01in{}%
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc|c}
\toprule[1pt]
Model & Config & Depth & mAP/mAR/Prec
% &  {\footnotesize{}{mAR@100}} & {\footnotesize{}{Prec@100}} 
\tabularnewline
\midrule[1pt]

% Image-based & - & 12 &  24.48 & 14.95  &  20.62  \\
% Text-based & - & 12  & 48.54  & 18.31  &  47.35 \\ \hline
w/o-Cross & (6,0,6) & 12 & 73.8 / 28.2 / 71.5 \\
w/o-Co & (6,6,0) & 12 & 73.2 / 29.3 / 72.8 \\  
% wo-Co\&Cross & (12,0,0) & 12 & 73.1 / 28.8 / 71.3  \\  
w/o-Txt/Vis & (0,6,6) & 12 &  69.3 / 25.4 / 68.4  \\
\midrule[0.7pt]
CAPTURE-A & (2,5,5) & 12 &  72.8 / 29.0 / 71.3   \\
CAPTURE-B & (5,2,5) & 12 & 73.7 / 29.1 / 71.8  \\
CAPTURE-C & (5,5,2) & 12 &  73.8 / 29.5 / 72.0  \tabularnewline
\midrule[0.7pt]
CAPTURE-S & (2,2,2) & 6 & 67.7 / 25.7 / 68.3 \\
CAPTURE-L & (8,8,8) & 24 &  74.7 / 30.9 / 74.2   \\
\midrule[0.7pt]
\textbf{CAPTURE} & \textbf{(4,4,4)} & \textbf{12} & \textbf{74.6 / 30.1 / 73.9} \\

\bottomrule[1pt]
\end{tabular}}
\caption{Performance of different layer configurations. 
Evaluation for $N=100$.}
\label{tab:ablation_layer}
\end{table}



\subsection{Impact of Layer Configuration}
\label{sec_layer_ablation}
We investigate how the configuration of transformer layers will affect the performance of our model in Table \ref{tab:ablation_layer}. 
The triplet in the Config column stands for the number of Text/Visual Transformer, Cross-Transformer, and Co-Transformer layer, respectively.
We first remove layers of a specific type while keeping the depth of the resulting network the same as CAPTURE's, i.e., 12 layers, for a fair comparison. 
The `w/o-Cross', `w/o-Co', and `w/o-Txt/Vis' refer to the resulting model after removing the Cross-Transformer, Co-Transformer, and Text/Visual Transformer layers from CAPTURE. 
As can be seen, the performances of these three models are inferior to that of CAPTURE, which demonstrates the effectiveness of its hybrid-stream architecture.
Moreover, in the second group of Table \ref{tab:ablation_layer} (CAPTURE-A,B,C), we study the combination of three layer types in different proportions. 
It turns out that the (4,4,4) configuration achieves the best performance. 
We further explore the performance of a smaller model (CAPTURE-S) and a larger model (CAPTURE-L). 
As can be seen, CAPTURE with the (4,4,4) configuration achieves a better trade-off between accuracy and parameters. 



\subsection{Zero-Shot Instance-Level Retrieval}
We argue that a retrieval-based solution generalizes better to real-world scenarios where the category set is updated continuously and large quantities of
 clean labels are too costly to collect. 
Unlike detection, our retrieval-based framework does not rely on a fixed-size collection of predefined classes or fine-grained box annotations.
To emphasize this, we conduct zero-shot retrieval experiments and report the results in Table \ref{tab:zero_shot}.
We manually remove 5/10/20 brands from the \textit{train} set and train CAPTURE on the remaining samples so that the removed categories are not disposed to our model during training. 
Then we evaluate CAPTURE on the classes of these unseen brands. 
We further compare our model with a two-stream model LXMERT and a single-stream model UNITER. 
As can be seen, CAPTURE achieves better performance than LXMERT and UNITER for all three metrics, which well demonstrates its generalization capacity.
We also visualize the embeddings generated by CAPTURE and UNITER via t-SNE \cite{van2008visualizing} in Figure \ref{fig_visualize}. 
It turns out that the features encoded by CAPTURE are more discriminative, which thus benefits the retrieval task.

\begin{table}
\centering
\setlength{\belowcaptionskip}{-0.3cm}
% \tabcolsep 0.01in{}%
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule[1pt]
 & Metric & $N=10$ &  $N=50$  \tabularnewline
\midrule[1pt]
\multirow{3}{*}{\rotatebox{90}{\scriptsize 5 brands}} & 
mAP$@N$ &  63.3 / 64.5 / \textbf{67.1} &  60.7 / 62.2 / \textbf{64.4}  \tabularnewline
& mAR$@N$ & 23.2 / 24.7 / \textbf{25.9}  &  19.2 / 20.1  / \textbf{20.9}   \tabularnewline
&Prec$@N$ & 56.5 / 57.1 / \textbf{60.5}  &  56.5 / 57.7 / \textbf{62.4}   \tabularnewline
\midrule[0.7pt]
\multirow{3}{*}{\rotatebox{90}{\scriptsize 10 brands}} &
mAP$@N$ & 56.8 / 58.2 / \textbf{61.5} &  54.1 / 55.2 / \textbf{57.1}   \tabularnewline
&mAR$@N$ & 19.6 / 20.5 / \textbf{24.0}  &  16.4 /17.4 / \textbf{18.4}   \tabularnewline
&Prec$@N$ & 50.2 / 51.9 / \textbf{53.0}  &  51.3 / 52.7 / \textbf{54.3}   \tabularnewline
\midrule[0.7pt]
\multirow{3}{*}{\rotatebox{90}{\scriptsize 20 brands}} 
& mAP$@N$ & 42.6 / 43.3 / \textbf{44.4}  & 36.7 / 37.3 / \textbf{38.8}   \tabularnewline
&mAR$@N$ & 17.5 / 17.6 / \textbf{17.9}  &  12.9 / 13.2 / \textbf{13.5}   \tabularnewline
&Prec$@N$ & 32.2 / 32.4 / \textbf{34.0}  &  32.9 / 33.1 / \textbf{34.5}  \tabularnewline
\bottomrule[1pt]
\end{tabular}}
\caption{Performance comparison of zero-shot retrieval. Organized in the order of LXMERT/UNITER/CAPTURE.}
\label{tab:zero_shot}
\end{table}


% \begin{table*}
% \centering
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule[1pt]
% Method& {\footnotesize{}{mAP@10}} & {\footnotesize{}{mAP@50}} & {\footnotesize{}{mAP@100}} & {\footnotesize{}{mAR@10}} & {\footnotesize{}{mAR@50}} & {\footnotesize{}{mAR@100}} & {\footnotesize{}{Prec@10}} & {\footnotesize{}{Prec@50}} & {\footnotesize{}{Prec@100}} \tabularnewline
% \midrule[1pt]

% CAPTURE_{wo MRM} & & & & & & & & &\\
% CAPTURE_{wo MLM} & & & & & & & &  \\  
% CAPTURE_{wo mask} & & & & & & & &  \\
% CAPTURE_{wo CRL} & & & & & & & &  \\
% CAPTURE_{w ITM} & & & & & & & &  \\

% \bottomrule[1pt]
% \end{tabular}
% \caption{Ablation study of multi-modal contrastive loss}
% \label{tab_performance}

% \end{table*}



\begin{table}
\centering
\setlength{\belowcaptionskip}{-0.3cm}
\footnotesize
% \tabcolsep 0.01in{}%
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc}
\toprule[1pt]
Method& {\footnotesize{}{mAP$@100$}} &  {\footnotesize{}{mAR$@100$}} &  {\footnotesize{}{Prec$@100$}} \tabularnewline
\midrule[1pt]
UNITER-single & 86.56 & 80.82 & 80.82 \tabularnewline
LXMERT-single & 86.05 & 80.59 & 80.59 \tabularnewline
CAPTURE-single & \textbf{88.24} & \textbf{83.33} & \textbf{83.33} \tabularnewline
\midrule[0.7pt]
CAPTURE-natural & 70.36 & 26.46 & 66.53 \tabularnewline
% Proposal-wise Retrieval &  73.78  & 29.21  & 72.87  \tabularnewline 
CAPTURE-1Inst  &  60.03 &   20.43 &  58.42  \tabularnewline
CAPTURE & \textbf{74.63} & \textbf{30.08} & \textbf{73.86}    \tabularnewline
\midrule[0.7pt]
% Image-level Retrieval & 27.84 &  44.51 &  29.07    \tabularnewline 
% CAPTURE &  67.40 &  62.46 &  66.19 \tabularnewline 
% \hline
CAPTURE-subset & 73.36  & 30.44 & 72.41 \tabularnewline
CAPTURE-gt & \textbf{77.79} & \textbf{37.40} & \textbf{77.13} \tabularnewline

% \hline
\bottomrule[1pt]
\end{tabular}}
\caption{Ablation study of single-product retrieval and the impact of detection performance on retrieval. Note that for single-product retrieval, the metric Prec$@N$ is equivalent to mAR$@N$ since there is only one category in an image.}
\label{tab:ablation_detector}
\end{table}



% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%             \toprule[1pt]
%             Method & {\footnotesize{}{Test set accuracy}} \\
%             \midrule[1pt]
%             VilBERT \cite{lu2019vilbert} & 97.06 \\
%             VL-BERT \cite{Su2020VL-BERT:} & 97.17 \\
%             VisualBERT \cite{li2019visualbert} & 97.49 \\
%             LXMERT \cite{tan2019lxmert} & 97.61 \\
%             UNITER \cite{chen2020uniter} & 97.67 \\
%             \textbf{CAPTURE (Ours)} & \textbf{97.78} \\
%             \bottomrule[1pt]
%     \end{tabular}
%     \caption{Classification results}
%     \label{tab:classification}
% \end{table}

% \FIXME{
% In the past few years, Bert has achieved significant performance on many natural language processing tasks, and there are also some methods that use Bert for text retrieval. For text retreival, Bert is pre-trained with all the titles and then finetuned with triplet loss which bring close the anchor with the positive as far as possible from the negative. Different from the supervised settting, examples of the same category can be selected as positive sample pairs, and examples of different categories can be selected as negative sample pairs. Here we use the text similarity to construct positive and negative sample pairs. Different from the natural text which contains rich contextual semantic information, the title of the product consists of some brand words and product words which contain less semantic information. So we use the jaccard similarity to calculate the similarity between titles. The sample with the strongest similarity is regarded as positive. For nagative, 100 samples are randomly selected to calculate the similarity, and the one with the worst similarity is regarded as a negative sample pair. The formulation is defined as:}
% \begin{equation}
%     L(a,p,n)=max(0,D(a,p)-D(a,n)+margin)
% \end{equation}




% \subsection{Effectiveness of inter-modal relations modeling}
% \label{sec_relation_ablation}
% Our proposed CAPTURE is able to model the inter-modal relations and capture the potential synergy between text and image, which is critical for multi-modal instance-level retrieval. 
% To verify this, we conduct several experiments to demonstrate the significance of relation modeling. 
% We first explore the effect of cross-transformer layers and co-transformer layers in Figure \ref{fig_overall_CAPTURE}(b).
% For the `CAPTURE-wo-CrossAttn' in Table \ref{tab_performance}, we remove the Text Cross-transformer and Visual Cross-transformer layers and report the results of this model. 
% For the `CAPTURE-wo-CoAttn' in Table \ref{tab_performance}, we remove the Text-visual Co-transformer layers.
% As can be seen, these two models are inferior to the full version of CAPTURE in terms of mAP, mAR, and Prec metrics, which suggests that the design of cross-modal attention and feature fusion module is critical for achieving good performance on our proposed task.

% Furthermore, we also compare the performance of our model with  ViLBERT \cite{lu2019vilbert}, the state-of-the-art multi-modal two-stream model,  and `ResNet-BERT' in Table \ref{tab_performance} and Figure \ref{fig_ap_ar_prec}.
% The main difference between CAPTURE and ViLBERT lies in the design of cross-modal relation modeling and feature fusion module, and it turns out that our CAPTURE surpasses ViLBERT in all metrics under the same training settings. 
% % As is described in Section \ref{sec_benchmark}, the main difference between CAPTURE and ViLBERT lies in the way of cross-modal relation modeling and cross-modal feature fusion, 
% % and it turns out that our CAPTURE surpasses ViLBERT in all metrics.
% For `ResNet-BERT' model, we adopt ResNet-50 \cite{he2016deep} pre-trained on ImageNet and BERT \cite{devlin2018bert} trained on the product titles of our dataset as the separate encoder for the image and text, respectively, and the input of retrieval is obtained by concatenating the outputs of two models. 
% Though these two models are the most prevailing networks for encoding images or texts, this hybrid model, however, achieves much worse performance compared to CAPTURE, which is not surprising since the cross-modal relation modeling mechanism is absent in this scheme. 
% Together with the results reported in Section \ref{sec_cross_comparison}, we conclude that cross-modal relation modeling and feature fusion play a critical role in our proposed task.
% We give detailed comparisons of CAPTURE and the baselines above in Figure \ref{fig_ap_ar_prec}, and our CAPTURE dominates these baselines in all three metrics.
% More comprehensive comparisons with other pre-trained multi-modal models can be found in the Supplementary Materials.







% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.92\textwidth]{latex/images/ap_ar_prec.pdf}
%     \caption{Precision, mAP, and mAR curves of different schemes compared to our CAPTURE.
%     The first row shows the comparisons between CAPTURE with two intra-modal retrieval baselines, i.e., Image-based Retrieval and Text-based Retrieval. 
%     The second row compares CAPTURE to several variants of itself and some prevailing visual-language models. 
%     Our CAPTURE dominates these baselines in all metrics.}
%     \label{fig_ap_ar_prec}
% \end{figure*}



\subsection{Comparisons on Single-Product Retrieval}
\label{sec_single_product_ablation}
It is noteworthy that CAPTURE is applicable to both single-product  and multi-product retrieval.
Indeed, it excels on these two tasks and achieves better performance than other baselines in single-product retrieval.
Specifically, for each single-product sample in the \textit{gallery} set, we pick it out as a query and perform single-product retrieval among the remaining samples in the \textit{gallery} set.
We compare the performance of three models, i.e., UNITER-single, LXMERT-single and CAPTURE-single, in Table \ref{tab:ablation_detector}. 
As can be seen, the performance of single-product retrieval is much higher than that of multi-product retrieval since the difficulty is largely reduced when there is only one instance/entity in the image/text. 
Furthermore, we notice the performance of `CAPTURE-single' is still better than that of two other baselines, which further demonstrates the superiority of CAPTURE.

\begin{figure}
% \setlength{\belowcaptionskip}{-0.6cm}
    \centering
    \includegraphics[width=0.5\textwidth]{images/embedding.pdf}
    \caption{Visualize the embeddings generated by CAPTURE and UNITER via t-SNE. 
    Points belonging to the same category are of the same color. Best viewed in color.}
    \label{fig_embedding}
\end{figure}

% To demonstrate the challenges of our proposed task compared with single-product retrieval, we randomly select 10\% single-product images as the query image (instead of multi-product query images) and report the results on the remaining single-product samples, referred as `Single-product Retrieval' in Table \ref{tab_imagelevel_gt}. 
% As can be seen, the performance of single-product retrieval is much higher than that of multi-product retrieval since the difficulty is largely reduced when there is only one instance/entity in the image/text. 
% Furthermore, we report the result of `Image-level Retrieval' scheme where the input to CAPTURE is an image and an image-level bounding box (of the same size as the image). 
\subsection{Impact of Detection Performance on Retrieval}
\label{sec_detector_ablation}
We conduct several experiments to explore how the performance of a detector will influence instance-level retrieval. 
The results are listed in Table \ref{tab:ablation_detector}.
As we claim in Section \ref{sec_rpn}, the off-the-shelf pretrained detectors are not readily applicable to our dataset due to the distribution difference between natural images and commodity images.
To verify this, we replace the RPN with Faster R-CNN \cite{ren2015faster} pre-trained on Visual Genome \cite{krishna2017visual} and utilize it to generate instance-wise input features of CAPTURE. 
The resulting model, named `CAPTURE-natural', is inferior to CAPTURE in all three metrics.
For the `CAPTURE-1Inst' model, we feed the whole image and an image-level bounding box, which is of the same size as the image, to CAPTURE for inference.
This scheme performs unsatisfactorily due to the failure of instance recognition, which suggests that the detector may become a performance bottleneck.
Going a step further, to explore the upper bound of CAPTURE, we randomly select 1,338 multi-product images and manually label the bounding boxes of these images. 
For the `CAPTURE-subset' model, we simply evaluate CAPTURE on this annotated subset. 
For the `CAPTURE-gt' model, the ground truth boxes and their corresponding features serve as the input to CAPTURE. 
As can be seen, the performance gap of these two models suggests that the performance of a detector can play an essential role in instance-level retrieval.
Moreover, the mAR gap between them is relatively large, which indicates that the false negatives in detection will hurt the performance of instance-level retrieval. 


% Furthermore, we explore the performance of two image-level retrieval schemes for the instance-level retrieval task.
% For `Proposal-wise Retrieval' in Table \ref{tab_imagelevel_gt}, we use bounding boxes detected by the RPN to extract instance features from ResNet backbone via RoI-Align \cite{he2017mask} and retrieve the corresponding single-products based on this set of features. 
% For `Single-instance Retrieval' in Table \ref{tab_imagelevel_gt}, we feed the whole image and an image-level bounding box, which is of the same size as the image, to our CAPTURE.
% These two schemes perform unsatisfactorily due to the failure of instance recognition, which suggests that the detector may become a performance bottleneck. 
% Thus we randomly select 1,338 multi-product images and manually label the bounding boxes of these images and these ground truths serve as the input of `CAPTURE-gt' in Table \ref{tab_imagelevel_gt}. 
% It achieves 66.01, 76.19, 61,61 in terms of $\mathrm{mAP}@100$, $\mathrm{mAR}@100$ and $\mathrm{Prec}@100$, respectively. 
% In comparison, we evaluate CAPTURE on this subset, referred as `CAPTURE-subset', and its performance is 2.04, 17.56, and 0.25 lower than `CAPTURE-gt' in terms of three metrics above. 
% As can be seen, the gap of the mAR metric between these two models is relatively large, which indicates that the missed detection by detector will harm the performance of instance-level retrieval. 
% \FIXME{CAPTURE-rcnn
% To demonstrate the importance of RPN in our model, we evaluate the CAPTURE which adopts a Faster-RCNN\cite{} pretrained on the Visual Genome
% dataset\cite{} to extract region feature, referred as 'CAPTURE-rcnn'.
% }
% Furthermore, we replace the RPN with Faster R-CNN \cite{ren2015faster} pre-trained on Visual Genome \cite{krishna2017visual}, which is a dataset with natural scene images, and compare their performance.
% This model, referred as `CAPTURE-rcnn', is also inferior to CAPTURE-subset, which demonstrates the effectiveness of the training process of our RPN detector.
% For more details, please refer to the Supplementary Materials.
% These experiments show that the performance of the detector is also an important factor for instance-level retrieval.



% \subsection{Generalization to unseen categories}
% \label{sec_generalize}
% Compared to a classification model, our retrieval scheme does not require class labels and a fixed category set. 
% % To demonstrate the generalization capacity of our retrieval model, we randomly choose \FIXME{20 classes} and train the `CAPTURE-generalize' model on the remaining data under the same setting.
% To demonstrate the generalization capacity of our retrieval model, we split the single-product set into two parts according to the brands of samples. 
% We train the `CAPTURE-generalize' model on 53-class LANCOME set (42,382 samples) and evaluate it on the remaining 20-class SKII set (26,121 samples) under the same settings.
% We compare the performance of CAPTURE and CAPTURE-generalize on these 20 SKII classes in Table \ref{tab_generalize}. 
% As can be seen, CAPTURE-generalize achieves satisfactory results in all metrics, which clearly demonstrates the extendibility of our framework.


\begin{figure}
% \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    \includegraphics[width=0.5\textwidth]{images/visualization.pdf}
    \caption{Visualizations of the retrieval results generated by CAPTURE. 
    Multi-product query images are on the left. 
    Correct/Incorrect retrieval images are highlighted in green/red boxes.
    }
    \label{fig_visualize}
\end{figure}




==> ex_introduction.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:intro}}

\IEEEPARstart{I}{n} the past twenty years, the commodity types have been richer than ever and the demand of online customers for E-commerce has wide been expanded. 
On the one hand, online merchandise has increasingly diversified categories and a large proportion of them are displayed as a product portfolio where multiple instances of different products exist in one image. On the other hand, online customers or merchants may want to find the single product in a portfolio for price comparison~\cite{vogler2016cancer} or online commodity recommendation~\cite{rahayu2017systematic}. Furthermore, as a result of increasing accumulation of heterogeneous data generated by shopping websites, it remains difficult to use an algorithm to handle large-scale and weakly annotated data~\cite{wang2016comprehensive} for multi-modal retrieval.

\begin{figure}[h]
% \setlength{\belowcaptionskip}{-0.6cm}
    \centering
    \includegraphics[width=0.5\textwidth]{images/instance_retrieval.pdf}
    \caption{
    % Comparisons of different retrieval paradigms. 
    Our proposed task performs \textbf{instance-level} retrieval among \textbf{multi-modal} data.}
    \label{fig_task_difference}
\end{figure}

\begin{table*}
\centering
\setlength{\belowcaptionskip}{-0.5cm}
% \tabcolsep 0.01in{}%
\begin{tabular}{c|cccc|ccc}
\toprule[1pt]
{{Dataset}}& {\footnotesize{}{\#samples}} &  {\footnotesize{}{\#categories}} &  {\footnotesize{}{\#instances}}
&  {\footnotesize{}{\#obj/img}} 
% &  {\footnotesize{}{full supervision}}
&  {\footnotesize{}{weak supervision}}
&  {\footnotesize{}{multi-modal}}
&  {\footnotesize{}{instance-level retrieval}}
\tabularnewline
\midrule[1pt]
RPC checkout \cite{wei2019rpc} & 30,000 & 200 & 367,935 & 12.26 &  & & \tabularnewline
Twitter100k \cite{hu2017twitter100k} & 100,000 & - & - & - & \checkmark &\checkmark & \tabularnewline
INRIA-Websearch \cite{Krapac2010ImprovingWI} &  71,478 & 353  & - & - &\checkmark &\checkmark & \tabularnewline
Dress Retrieval \cite{corbiere2017leveraging} & 20,200 & - & $\sim$20,200 & $\sim$1.0&\checkmark &\checkmark & \tabularnewline
% \hline
% Product1M-gallery (Ours) & 40,033 & 458 & 40,033 & 1 & \checkmark& \checkmark & \checkmark \tabularnewline
% Product1M-query (Ours) & 9,220 & 392 & 26097 & 2.83 & \checkmark & \checkmark  &\checkmark \tabularnewline
\textbf{Product1M(Ours)} & \textbf{1,182,083}  & \textbf{458} & \textit{92,200} & \textit{2.83} & \checkmark & \checkmark  & \checkmark \tabularnewline

\bottomrule[1pt]
\end{tabular}
\caption{Comparisons between different datasets. `-' indicates inapplicable. The \#instances and \#obj/img of Product1M are in italics since there are no instance labels for the \textit{train} set and we only count the instances in the \textit{val} and \textit{test} set. Product1M is one of the largest multi-modal datasets as well as the first dataset specifically tailored for real-world instance-level retrieval scenarios.}
\label{tab_statistics}
\end{table*}

In this paper, we investigate a realistic problem: \textit{how to perform instance-level\footnote{Instance-level product retrieval refers to the retrieval of all single products existed in a product portfolio image.} fine-grained product retrieval given the large-scale weakly annotated multi-modal data?} 
We compare different retrieval patterns in Figure \ref{fig_task_difference}. 
As can be seen, image-level retrieval tends to match the  results from the whole aspact since it does not distinguish different instances, while multi-modal instance-level retrieval is more favorable for searching for various kinds of products among multi-modal data. 
Despite the generality and the practical value of this problem, it is not well studied due to the lack of real-world datasets and a clear problem definition.
In the literature of product retrieval, intra-modal \cite{qi2016sketch,bai2018optimization,qayyum2017medical,nurmi2008product} and cross-modal retrieval \cite{wang2017adversarial,feng2014cross,wei2016cross,cao2016deep,wang2015joint,deng2018triplet} take as input single-modal information, e.g., an image or a piece of text, and performs matching search between separate data points.
Unfortunately, such retrieval schemes significantly restrict their use in many scenarios where multi-modal information exists in both the queries and targets.
More importantly, previous works focus on the relatively simple case, i.e., image-level \footnote{Image-level product retrieval refers to recognizing a specific product instance in a single-product image.} retrieval for single-product images \cite{kuang2019fashion,gu2018multi} and the instance-level nature of retrieval is unexplored. 

To bridge this gap and advance the related research, we collect a large-scale dataset, named Product1M, proposed for multi-modal instance-level retrieval.
%and propose a novel self-training framework that extracts representative features from noisy multi-modal data to perform instance-level product retrieval. 
Product1M contains over 1 million image-caption pairs and consists of two types of samples, i.e., single-product and multi-product samples. 
Each single-product sample belongs to a fine-grained category and the inter-category difference is subtle. 
The multi-product samples are of great diversity, resulting in complex combinations and fuzzy correspondence that well mimic the real-world scenarios.
% Each single-product sample belongs to a fine-grained category and the inter-category difference is subtle, which poses challenges to the retrieval framework. 
% The multi-product samples are crawled on E-commerce websites and have complex combinations of multiple single-products and different types of noises are presented to mimic the real-world instance-level retrieval scenarios.
To the best of our knowledge, Product1M is one of the largest multi-modal datasets as well as the first dataset specifically tailored for real-world  multi-modal instance-level retrieval scenarios.
% We provide some samples to demonstrate the characteristics of our dataset in Figure \ref{} and challenges that need to be solved are illustrated in Section \ref{sec_challenge}. 

In addition to the constructed dataset, we also propose a novel self-supervised training framework that extracts representative instance-level features from large-scale weakly annotated data. 
% In contrast, many previous approaches \cite{corbiere2017leveraging,wei2019rpc} rely on coarse- or fine-grained annotations to train a deep neural network and have poor scalability with respect to the massive amount of noisy weakly annotated data in the real-world database. 
% Cross modal pretraining
Specifically, we first train a multi-product detector from pseudo-labels by incorporating a simple yet effective data augmentation scheme. 
Then, CAPTURE is proposed to capture the potential synergy of images and texts via several pretext tasks. 
We showcase that some prevailing cross-modal pretraining methods \cite{lu2019vilbert,li2019visualbert,chen2020uniter,tan2019lxmert} might be flawed under the multi-instance setting due to the design defects in the network architecture or the inappropriate pretext task.
In contrast, CAPTURE utilizes a hybrid-stream architecture that encodes data of different modalities separately and fuses them in a unified way, which is experimentally shown to be beneficial for our proposed task. 
Moreover, we introduce the cross-modal contrastive loss to enforce CAPTURE to reach alignment between image and texts, which avoids the mismatch issue incurred by the inappropriate pretext task.

% \textbf{Single-Product Samples}
% We show some single-product images in Figure ~\ref{fig:fig_SP_images}  and captions are not included for simplicity. 
% The inter-category differences are subtle and some products of different categories have almost the same appearance except that the words on the packing are slightly different.
% \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\textwidth]{images/visualize1.png}
%     \caption{Single-product samples.}
%     \label{fig:fig_SP_images}
% \end{figure*}





% \textbf{Multi-Product Samples}
% Figure ~\ref{fig:fig_MP_images} shows some multi-product images and captions are not included for simplicity. 
% As can be seen, the combinations of single-product are complicated and
% noises like irrelevant objects, watermarks and complex background are widely existed.
% \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\textwidth]{images/visualize2.png}
%     \caption{Multi-product samples.}
%     \label{fig:fig_MP_images}
% \end{figure*}

% To further discriminate different instances in an image, we decouple instances from an image and construct positive pairs among image, instances and text for unsupervised contrastive learning. 

Crucially, CAPTURE surpasses the SOTA cross-modal baselines in terms of all main metrics by a large margin. 
We further conduct extensive ablation experiments to demonstrate the generalization capacity of CAPTURE and explore several critical factors of our proposed task. 
We hope the proposed Product1M, CAPTURE, and solid baselines can help advance future research on real-world retrieval.

\begin{figure*}
\setlength{\belowcaptionskip}{-0.6cm}
    \centering
    \includegraphics[width=1.0\textwidth]{images/challenges_statistics.pdf}
    \caption{Characteristics and statistics of Product1M: (1a) Complex combinations of single-product; (1b) Weak supervision and fuzzy correspondence; (1c) Difficulties in real-world scenarios; 
    (2) Long-tailed category distribution of Product1M. The line displays the sample number of each category in decreasing order. Product1M contains a wide variety of categories and the long-tailed class distribution aligns well with real-world scenarios.}
    \label{fig_challenge_statistics}
\end{figure*}


==> ex_method.tex <==
\section{Methodology}\label{sec:method}

As is depicted in Figure \ref{fig_overall_CAPTURE}, our framework consists of an augmentation-based detector and a self-supervised multi-modal transformer. 
In this section, we first elaborate the training process of RPN and the architectural design of CAPTURE in Section \ref{sec_rpn} and Section \ref{sec_CAPTURE_arch}. 
Then we describe two kinds of pretext tasks that enables the self-supervised learning of CAPTURE in Section \ref{sec_capture_masked} and Section \ref{sec_capture_contrastive}. 
Finally, we illustrate the inference process for instance-level retrieval in Section \ref{sec_inference}.

\subsection{Training RPN for Multi-Product Detection}
\label{sec_rpn}
Retrieval based simply on the image-level features will lead to an undesirable condition where the retrieval results are overwhelmed by the dominated product in an image.
Thus it is crucial to distinguish different products and extract proposal-wise features in a multi-product image.
% \ycnote{Single-images with clean background are actually used to generate synthetic data.}
While many pre-trained detectors are available, they are infeasible to directly apply to multi-product detection due to the distribution difference between datasets. 
Thus we utilize a simple yet effective data augmentation scheme to train a Region Proposal Network (RPN) \cite{ren2015faster} based solely on the single-product images as shown in Figure \ref{fig_overall_CAPTURE}(a). 
We first use GrabCut \cite{Meng2014GrabCut} to obtain the foreground masks of single-product images.
With real-world background images from Places365 \cite{zhou2017places}, a copy-and-paste augmentation \cite{dwibedi2017cut} is applied to these foreground masks and background images to generate synthesized images. 
In this way, we are able to train a well-performing multi-product detector.
% that achieves 96\% Average Recall. 
Given the detected regions of RPN, we utilize RoIAlign \cite{he2017mask} to obtain instance-wise features, which are then fed into CAPTURE for further cross-modal learning. 
More visualizations and details about the synthesized images and the training of RPN can be found in the Supplementary Materials. 


\subsection{Architectural Design of CAPTURE}
\label{sec_CAPTURE_arch}
After training the RPN, we can generate high-quality proposals for different products in an image. 
% Vision-language pre-trained models  \cite{lu2019vilbert,Su2020VL-BERT:,li2019visualbert,chen2020uniter} have demonstrated the state-of-the-art results in a variety of downstream tasks. 
Different from the prevalent single-stream or two-stream transformer architectures, we propose CAPTURE that combines these two architectures into a unified one by stacking three types of layers for semantic alignment and joint learning of multi-modal inputs.
Details are shown in Figure \ref{fig_overall_CAPTURE}(b). 
To be specific, the Text/Visual Transformer takes as input the embeddings of the texts or image and is responsible for intra-modal feature learning. 
The Text/Visual Cross-Transformer aims to capture and model the inter-modal relations between texts and image by exchanging key-value pairs in the multi-headed attention mechanism.
% , which helps to refine the mid-level representations of different modalities mutually. 
After that, the features of texts and image are concatenated and serve as the query, key, and value inputs to the Co-Transformer for joint learning of multi-modal features. 
These three types of transformer are stacked $L, K$, and $H$ times respectively. 
We verify the effectiveness of our architectural design in Table \ref{tab:ablation_layer}.
% \begin{table*}[h]
% \centering
% % \tabcolsep 0.01in{}%
% \resizebox{\textwidth}{20mm}{
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule[1pt]
% Method& {\footnotesize{}{mAP@10}} & {\footnotesize{}{mAP@50}} & {\footnotesize{}{mAP@100}} & {\footnotesize{}{mAR@10}} & {\footnotesize{}{mAR@50}} & {\footnotesize{}{mAR@100}} & {\footnotesize{}{Prec@10}} & {\footnotesize{}{Prec@50}} & {\footnotesize{}{Prec@100}} \tabularnewline
% \midrule[1pt]

% Image-based Retrieval & 27.31 &  27.17 &  27.84 & 24.52 & 39.19 & 44.51 & 25.74 &  27.24 & 29.07   \tabularnewline 
% Text-based Retrieval &  58.53 &  52.93 &  50.79 & 48.16 & 56.24 & 61.27 & 49.84 & 46.70 & 45.92 \tabularnewline 
% \hline
% ViLBERT \cite{lu2019vilbert} & 59.51 &  57.31 &  56.38 & 45.81 & 54.34 & 57.47 & 53.57 & 54.97 & 54.84 \tabularnewline 
% ResNet-BERT \cite{he2016deep,devlin2018bert} & 36.33 & 35.03 & 33.77 & 22.21 & 47.18 & 57.53 & 20.80 & 28.38 & 30.86 \tabularnewline
% % \hline
% % Image-level Retrieval &  37.86 & 37.01 &  37.60 & 29.31 & 43.60 & 47.72 & 30.94 & 35.67 & 37.49 \tabularnewline 
% % Single-instance Retrieval & 60.29 &  58.56 &  57.69 &  43.50 &  47.69 &  49.90 &  67.30 & 68.66  & 68.72  \tabularnewline 
% \hline
% CAPTURE-wo-CrossAttn & 50.13 & 55.48 & 52.17 & 37.40 & 45.11 & 50.98 & 50.13 & 53.22 & 52.20  \tabularnewline 
% CAPTURE-wo-CoAttn & 61.94 & 61.02 & 60.58 & 43.24 & 55.53 & 60.82 &  51.59 & 57.79 & 58.65 \tabularnewline 
% \hline
% \textbf{CAPTURE (Ours)} & \textbf{70.69} & \textbf{68.22} & \textbf{67.40} & \textbf{48.26} &  \textbf{59.23} & \textbf{62.46} & \textbf{60.64} & \textbf{65.90} & \textbf{66.19}   \tabularnewline
% \bottomrule[1pt]
% \end{tabular}}
% \caption{Performance of different schemes for weakly-supervised multi-modal instance-level retrieval.}
% \label{tab_performance}
% \end{table*}




% new table 








% To be specific, the Transformer layer can be denoted as below:
% \begin{equation}
%     \operatorname{Attention}(Q, K, V)=\operatorname{Softmax}\left(QK^{T} / \sqrt{d}\right) V,
% \end{equation}
% where $Q, K, V$ stand for query, key, value and $d$ is the dimension of inputs.

% there are three different types of layers in CAPTURE, including vanilla transformer, cross-transformer, and co-transformer. 


\begin{table*}[h]
\centering
% \setlength{\belowcaptionskip}{-0.6cm}
% \tabcolsep 0.01in{}%
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule[1pt]
Method& {\footnotesize{}{mAP@10}} & {\footnotesize{}{mAP@50}} & {\footnotesize{}{mAP@100}} & {\footnotesize{}{mAR@10}} & {\footnotesize{}{mAR@50}} & {\footnotesize{}{mAR@100}} & {\footnotesize{}{Prec@10}} & {\footnotesize{}{Prec@50}} & {\footnotesize{}{Prec@100}} \tabularnewline
\midrule[1pt]

% ViLBERT_{NA} \cite{lu2019vilbert} & 55.07  & 53.29    &  53.55  & 41.58  & 39.53  & 38.62  & 50.77  & 51.59  &  51.42 \\ 
% VL-BERT_{NA} \cite{lu2019vilbert} & 57.40  &  54.13  & 54.79   & 42.35  & 41.76  &  40.08 & 52.79   & 52.91  &  53.08 \\ 
% VisualBERT_{NA} \cite{lu2019vilbert} & 56.81  & 53.71   &  53.80  & 41.74  & 39.92  & 38.69  & 52.00  & 52.32  & 52.66  \\
% UNITER_{NA} \cite{lu2019vilbert} & 58.38  & 56.45   &  56.03  &  42.68 & 41.44  & 40.95  & 53.74  & 53.42  & 53.82  \\ 
% LXMERT_{NA} \cite{lu2019vilbert} & 58.07  &  55.86  &  55.42  & 42.60  &  40.92 & 39.83  & 52.39  & 53.64  & 53.89  \\ 
% \textbf{CAPTURE (Ours)} & \textbf{61.90} & \textbf{59.92} & \textbf{58.38} & \textbf{43.53} &  \textbf{41.74} & \textbf{40.92} & \textbf{55.46} & \textbf{56.28} & \textbf{56.53}   \tabularnewline
% \midrule
\textit{Image-based} & 40.35  &  36.77  & 34.76   & 17.20  & 15.86  & 15.45  & 32.80  & 30.54  & 29.97  \\

\textit{Text-based} & 61.56 &  59.38  & 58.42   & 23.65  & 22.04  & 20.13  & 56.15  & 57.47  & 57.45  \\
ViLBERT \cite{lu2019vilbert} & 70.11  &  68.19  &  68.29  &  29.05 & 25.54  & 25.02  &  64.64 & 66.35  &  66.60 \\
LXMERT \cite{tan2019lxmert} & 71.37  & 67.83   &  66.73  & 29.83  & 23.15  &  23.89 & 65.97  &  64.79 & 64.77  \\ 
CLIP* \cite{radford2021learning}  & 70.25  & 69.28   &  67.30  &  29.45  &  25.61  & 25.61 & 67.77  &  68.00 & 68.38 \\
VL-BERT \cite{Su2020VL-BERT:} & 72.01  & 68.22   & 67.79   &  29.15 & 25.59  & 26.16  &  65.25 & 66.92  & 66.64  \\ 
VisualBERT\cite{li2019visualbert} &  72.27 & 69.60   &  68.28  & 31.69  &  26.31 & 26.83  & 67.31  &  66.48 &  66.62 \\

UNITER \cite{chen2020uniter} & 74.69  & 71.02   &  70.93  &  29.47 & 25.82  &  26.20 & 70.11  &  69.15 & 68.95  \\

\textbf{CAPTURE (Ours)} & \textbf{79.36} & \textbf{74.79} & \textbf{74.63} & \textbf{34.69} &  \textbf{30.04} & \textbf{30.08} & \textbf{73.97} & \textbf{72.12} & \textbf{73.86}   \tabularnewline
\bottomrule[1pt]
\end{tabular}}
\caption{Comparison with different intra- and cross-modal self-supervised baselines.}
\label{tab_performance}
\end{table*}

\subsection{CAPTURE by Masked Multi-Modal Learning}
\label{sec_capture_masked}
We utilize several pretext tasks to enable the self-supervised learning of CAPTURE. 
For modality-wise feature learning, we adopt two masked multi-modal modeling tasks, i.e., Masked Language Modeling task (MLM) and Masked Region Prediction task (MRP), following the standard BERT \cite{devlin2018bert} and VisualBERT \cite{li2019visualbert}. 
Concretely, for MLM and MRP, approximately 15\% of texts and proposal inputs are masked out and the remaining inputs are used to reconstruct the masked information. 
The MLM is handled as in BERT \cite{devlin2018bert}.
For the MRP, the model directly regresses the masked features, which is supervised by the features extracted by the pretrained RPN with a MSELoss.
% --we use feature logically regression(MSE) but not class distributions. }
As for inter-modal relation modeling, Image-Text Matching task (ITM) is widely adopted in many previous methods \cite{li2019visualbert,chen2020uniter,lu2019vilbert,tan2019lxmert}. 
Typically, the model is asked to predict whether the text is the corresponding description of an image, which is formulated as a binary classification task.
To generate negative samples, either the image or caption is randomly substituted.
We argue that ITM could be problematic to the fine-grained understanding of an image-text sample at the instance-level. 
We hypothesize the deterioration stems from the unmatched image and caption pairs after substitution, which results in the inconsistency between detected regions and text. 
We further experimentally validate this claim in Table \ref{tab:loss_ablation}.

\subsection{CAPTURE by Cross-Modal Contrastive Loss}
\label{sec_capture_contrastive}
Aside from intra-modal feature learning, CAPTURE is expected to generate coherent representations of multi-modal inputs and learn the correspondence between them. 
To this end, we resort to inter-modality contrastive learning \cite{chen2020simple,radford2021learning} to reach alignment between image and text. 
For a minibatch of $N$ image-text samples, there are $2N$ data points in total.
We treat the corresponding image-text pairs as $N$ positive pairs, and the other $2(N-1)$ unmatched pairs are regarded as negative ones.
Formally, given an image-text pair $(x_i,x_j)$ and their encoded features $(\tilde{x}_i, \tilde{x}_j)$, the cross-modal contrastive loss for this positive pair is computed as:
\begin{equation}
   \mathcal{L}(x_i, x_j)=-\log \frac{\exp \left(\operatorname{sim}\left(\tilde{x}_i, \tilde{x}_j\right) / \tau\right)}{\sum_{k=1}^{2 N} \mathbbm{1}_{[k \neq i]} \exp \left(\operatorname{sim}\left(\tilde{x}_i, \tilde{x}_k\right) / \tau\right)},
\end{equation}
where $\operatorname{sim}(\boldsymbol{u}, \boldsymbol{v})=\boldsymbol{u}^{\top} \boldsymbol{v} /\|\boldsymbol{u}\|\|\boldsymbol{v}\|$ computes the cosine similarity of $(\boldsymbol{u}, \boldsymbol{v})$ pairs, $\tau$ denotes the temperature parameter, $\mathbbm{1}_{[k\ne i]}$ is a binary indicator function that returns 1 iff $k \ne i$.
% $\mathcal{Z}$ consists of three types of negative pairs:
% \begin{equation}
%     \mathcal{Z} = \sum_{k=1}^{N} \exp (\frac{\operatorname{sim}(\tilde{x}_i, \tilde{c}_k)}{\tau}) + 
%     \mathbbm{1}_{[k\ne i]}\exp (\frac{\operatorname{sim}(\tilde{x}_i, \tilde{x}_k)}{\tau}) + 
%     \mathbbm{1}_{[k\ne i]}\exp (\frac{\operatorname{sim}(\tilde{c}_i, \tilde{c}_k)}{\tau})
% \end{equation}
This form of contrastive loss  encourages the encoded features of positive pairs from different modality to be similar while discriminates those of negative ones. 
We find it beneficial to inject this supervision at the Text/Visual Transformer and further discussion about the effect of cross-modal contrastive loss can be found in Section \ref{sec_pretext_ablation}.



% In this way, we are able to generate unified, coherent, and discriminative features for an image-text pair that further boost the performance of retrieval. 
% The input to CAPTURE is an image-text pair with proper positional embeddings and segment embeddings \cite{devlin2018bert} for text and image. 
% Thanks to the high-quality proposals generated by the RPN, CAPTURE is aware of the existence of different instances and can encode both the appearance and positional features of them. 
% Crucially, the features of different regions are randomly masked to zero at a probability of 15\%, which benefits the self-supervised learning of CAPTURE. 
% We utilize three prevailing pretext tasks, i.e., ITM \cite{chen2020uniter}, Mask LM \cite{devlin2018bert}, Mask Region Predictions \cite{chen2020uniter}, for the self-training of CAPTURE.






% \subsection{Retrieval using pre-trained features}
\subsection{Inference for Instance-Level Retrieval}
\label{sec_inference}
% \FIXME{How to extract features***?}
% \FIXME{For single-product samples, we feed the image and the corresponding text into CAPTURE while the multi-product images are first feed into a trained RPN for object separation and then extract features via CAPTURE}
% Under the supervision of several pretext tasks as well as the cross-modal contrastive loss, CAPTURE is able to extract instance-wise features given the image-text pair of a portfolio. 
For both the single- and multi-product samples, the proposal-wise features extracted via the pre-trained RPN and the captions are used as input to CAPTURE.
During inference, the Co-Transformer layer outputs $H_{IMG}$ and $H_{TXT}$ as the overall representations of visual and linguistic inputs, respectively. 
These two vectors are multiplied together to derive the joint representations of an instance. 
Furthermore, since Text/Visual Transformer is supervised with cross-modal contrastive loss, we find it beneficial to concatenate the features of this layer for retrieval. 
The resulting features then serve as the input of our retrieval algorithm.
% The outputs of the co-transformer at the last layer serve as the input of our retrieval algorithm.
After computing the cosine similarity matrix between an instance and the samples in the $gallery$ set, we retrieve the corresponding single-product samples with the highest similarities for each query. 


==> ex_relatedwork.tex <==

\section{Related Work}\label{sec:related_work}

\noindent \textbf{Related Datasets}. \noindent\textbf{RPC} \cite{wei2019rpc} contains 53,739 single-product exemplar images and 30,000 checkout images. 
    Three different granularities of annotations are provided including category information, point-level annotations, and bounding boxes. 
    However, there exists a gap between RPC and real-world scenarios since RPC was captured under a controlled environment and no textual information is available in this dataset.
    
\noindent\item \textbf{Twitter100k} \cite{hu2017twitter100k} is proposed for weakly supervised cross-media retrieval. 
It contains 100k image-text pairs crawled from Twitter. There is no constraint for the categories of images and the text is written in informal language by users.
Similarly, this dataset focuses on image-level retrieval and use single-modal input as the query, which is not suitable for instance-level multi-modal retrieval. 

    % \item \textbf{RP2K} \cite{peng2020rp2k}
    % a large-scale retail product dataset for fine-grained product classification. 
    % It contains images of 2000 different products captured in real retail stores, each category has 250 images on average. 
    % Annotations with different granularities including sizes, shapes and flavors/scents are provided. 
    % This dataset focuses on image-level product information retrieval in retailing industry and multi-modal information like text is not taken in account. 
    
\noindent\textbf{INRIA-Websearch} \cite{Krapac2010ImprovingWI} is a cross-modal retrieval dataset that contains 71,478 image-text pairs with 353 different search queries, including actors, films, etc. 
    The images are collected via internet search and textual information consists of text surrounding images on websites. 
    % There are about 80\% of textual queries that correspond to more than 200 top-ranked images returned by the web search engine. 
    Cross-modal retrieval algorithms are performed on this dataset to solve the text-to-image searching problem.
    
\noindent\textbf{Dress Retrieval} proposed in \cite{corbiere2017leveraging} collects noisy labeled data crawled on E-commerce website catalogs. 
    Each fashion image is associated with some selected relevant fields filtered by predefined vocabulary. 
    Typically, each image contains a single instance, e.g., a model wearing a dress and the background is relatively clean. 

In comparison, our Product1M differs notably in four aspects from the above datasets:
\begin{itemize}
    \item Product1M is the first dataset tailored for instance-level retrieval, which is of great potential in E-commerce industry.
    \item Product1M extends the canonical intra- and cross-modal retrieval to multi-modal retrieval, where images and texts exist both in the query and the target. This is a more practical setting since the multi-modal information is ubiquitous in real world scenarios.
    \item The weakly annotated samples of Product1M enforces the model to excavate useful features without clean labels, which endows the model with great generalization capacity to large-scale and noisy data.
    \item Product1M is one of the largest datasets for retrieval and the product samples are of great diversity and well aligns with E-commerce industry.
\end{itemize}

\noindent\textbf{Intra- and Cross-Modal Retrieval.} Intra-modal retrieval \cite{qi2016sketch,bai2018optimization} has been extensively studied in the keyword-based web document retrieval \cite{ensan2017document}, content-based image retrieval \cite{noh2017large}, 
% medical image retrieval \cite{qayyum2017medical} 
and product recommendation \cite{kang2017visually,kang2019complete}. 
Cross-modal retrieval \cite{wang2017adversarial,feng2014cross,wei2016cross,cao2016deep,wang2015joint,deng2018triplet} emerges as a promising avenue for efficient indexing and searching among large-scale data with different modalities, and is widely used in search engines \cite{buttcher2016information,harman2019information}, E-commerce \cite{ji2017cross,corbiere2017leveraging}, to name a few.
However, these approaches \cite{nurmi2008product,lin2018regional,corbiere2017leveraging,wei2019rpc,wang2016effective} are typically subject to single modal inputs, which makes them hard to apply to many real-world scenarios where multi-modal information exists in both the queries and targets. 




\noindent\textbf{WSOD: Weakly Supervised Object Detection.} WSOD \cite{tang2018pcl,2018Generative,2019Cap2Det} reduces its excessive reliance on fine-grained labels by learning from cheaper or freely-available data. 
PCL \cite{tang2018pcl} iteratively generates proposal clusters to facilitate the learning of instance classifiers. 
Pseudo labels generated from image labels \cite{2018Generative} and unstructured textual descriptions like captions \cite{2019Cap2Det} are also beneficial for boosting the performance of WSOD. 
However, WSOD typically relies on a fixed-size collection of predefined classes and is not readily applicable to our proposed task where class labels are not available and categories can be updated dynamically.

\noindent\textbf{Cross-Modal Self-Supervised Learning.}
% Most related to our work is the concurrent transformer-based models for cross-modal self-supervised learning. 
Existing Vision-language pre-trained models typically use a multi-layer Transformer \cite{vaswani2017attention} architecture such as BERT \cite{devlin2018bert} to learn image-text semantic alignment on multi-modal data.
Single-stream models \cite{li2019visualbert,Su2020VL-BERT:,chen2020uniter} encode the combined multi-modal features in a unified architecture while other two-stream models \cite{lu2019vilbert,tan2019lxmert} instead utilize different encoders for inputs of different modalities. 
These methods are not tailored for instance-level retrieval  and we showcase that they might be flawed due to the design defects in the network architecture and the inappropriate pretext tasks. 





% \section{Product1M: Towards Combination-to-Single Product Retrieval}
\section{Instance-Level Retrieval on Product1M}
\subsection{Task Definition}
\label{sec_task_definition}

% We define the weakly-supervised instance-level retrieval problem as follows. 
A product sample $(I, C)$ is an image-text pair where $I$ is the product image and $C$ is the caption.
    Given the \textit{gallery} set of single-product samples $\mathcal{S}=\{\mathcal{S}_i |\mathcal{S}_i= (I_\mathcal{S}^i,C_\mathcal{S}^i)\}$ and the set of multi-product samples $\mathcal{P}=\{\mathcal{P}_i | \mathcal{P}_i=(I_\mathcal{P}^i,C_\mathcal{P}^i)\}$, the task is to retrieve and rank the single-products that appear in the query sample $\mathcal{P}_i$, i.e., to predict a list $RETR^i = [id^i_1, id^i_2, \cdots, id^i_k, \cdots, id^i_N]~~ \forall \mathcal{P}_i \in \mathcal{P}$, where $id^i_k$ corresponds to a specific single-product sample in $\mathcal{S}$.



\subsection{Dataset Statistics}
\label{sec_statistics}
We collect a large number of product samples of 49 brands from E-commerce websites.
These image-text samples are then manually divided into the single-product and multi-product groups according to the corresponding product information.
Product1M is split into the \textit{train}, \textit{val}, \textit{test}, and \textit{gallery} set. 
The \textit{train} set contains 1,132,830 samples including both the single-product and multi-product samples, while there are only multi-product samples in the \textit{val} and \textit{test} set, which contain 2,673 and 6,547 samples respectively.
The \textit{gallery} set has 40,033 single-product samples for 458 categories, 392 of which appear in the \textit{val} and \textit{test} set and the remaining ones act as interference items for validating the robustness of a retrieval algorithm.
% Each sample except for those in the \textit{train} set is annotated with class labels for the purpose of evaluation, i.e., they are not involved in the training process. 
The samples in the \textit{gallery}, \textit{val}, and \textit{test} sets are annotated with class labels for the purpose of evaluation, i.e., they are not involved in the training process, and the samples in the \textit{train} set are not annotated.
The statistics of Product1M are shown in Table \ref{tab_statistics} and Figure \ref{fig_challenge_statistics}. 


More visualizations of Product1M and comparisons with related datasets can be found in the Supplementary Materials.

\begin{figure*}
\setlength{\belowcaptionskip}{-0.6cm}
    \centering
    \includegraphics[width=1.0\textwidth]{images/overall.pdf}
    \caption{An overview of our instance-level retrieval pipeline. (a) Pretrain an RPN based on pseudo-labels generated by a copy-and-paste data augmentation scheme. (b) Utilize CAPTURE to capture the potential synergy across modality via a hybrid-stream architecture and several pretext tasks. (c) Construct positive pairs of matched image-text samples for cross-modal contrastive learning. Best viewed in color.}
    \label{fig_overall_CAPTURE}
\end{figure*}

\subsection{Dataset Characteristics}
\label{sec_challenge}


\noindent \textbf{Multi-product nature and complex combinations:} 
The multi-product images are ubiquitous on E-commerce websites and serve as the query images of instance-level product retrieval. 

As is shown in Figure \ref{fig_challenge_statistics}(1a), products can be organized in abundant forms and layouts and the number of instances can be large.
The excessive amount and great diversity of fine-grained single-product samples give rise to the complex combinations in different portfolio images.
    
\noindent \textbf{Weak supervision and fuzzy correspondence:}
    % We compare weakly-supervised retrieval on multi-modal data with other methods in Figure \ref{fig_comp}. 
    We consider using data of two common modalities, i.e., images and texts, for retrieval. 
    Unlike other datasets with clean class labels, 
    % or attribute annotations, 
    the supervision from commodity captions is weak and often uninformative. 
    We show different types of challenging samples in Figure \ref{fig_challenge_statistics}(1b).
    Some samples contain abbreviations, i.e., a shortened form of several products, in their captions.
    However, the abbreviation like `eight-piece set' does not contain any specific information about products.
    The second type of sample carries irrelevant information, where the commodities described in the title may not appear in the image or vice versa. 
    The wide distribution of fuzzy correspondence between images and titles makes it even more challenging for instance-level retrieval.

    
    
\noindent \textbf{Consistency with real-world scenarios:}
    We show some challenging samples in Figure \ref{fig_challenge_statistics}(1c). 
    They can have a complex background with irrelevant objects, amorphous watermarks, or significant clutter covering the product information. 
    Some products of different categories can have almost the same appearance except that the words on the packing are slightly different, e.g., \textit{day cream} vs \textit{night cream}. 
    As is shown in Figure \ref{fig_challenge_statistics}(2a,2b), the long-tailed distribution of Product1M aligns well with real-world scenarios.





